DeepSpeed Inference: Enabling Efficient Inference of Transformer Models at Unprecedented Scale

The past several years have witnessed the success of transformer-based models, and their scale and application scenarios continue to grow aggressively. The current landscape of transformer models is increasingly diverse: the model size varies drastically with the largest being of hundred-billion parameters; the model characteristics differ due to the sparsity introduced by the Mixture-of-Experts; the target application scenarios can be latency-critical or throughput-oriented; the deployment hardware could be single- or multi-GPU systems with different types of memory and storage, etc. With such increasing diversity and the fast-evolving pace of transformer models, designing a highly performant and efficient inference system is extremely challenging. In this paper, we present DeepSpeed Inference, a comprehensive system solution for transformer model inference to address the above-mentioned challenges. DeepSpeed Inference consists of (1) a multi-GPU inference solution to minimize latency while maximizing the throughput of both dense and sparse transformer models when they fit in aggregate GPU memory, and (2) a heterogeneous inference solution that leverages CPU and NVMe memory in addition to the GPU memory and compute to enable high inference throughput with large models which do not fit in aggregate GPU memory. DeepSpeed Inference reduces latency by up to 7.3X over the state-of-the-art for latency-oriented scenarios and increases throughput by over 1.5x for throughput-oriented scenarios. Moreover, it enables trillion parameter scale inference under real-time latency constraints by leveraging hundreds of GPUs, an unprecedented scale for inference. It can inference 25x larger models than with GPU-only solutions, while delivering a high throughput of 84 TFLOPS (over $50\%$ of A6000 peak).

==> inference-kernel-results.tex <==

\subsection{Performance Evaluation of Inference Kernels}\label{sec:kernel-evaluation}
\label{subsec:moe-perf}

In this section, we evaluate the performance of inference-optimized kernels using single-GPU 
and multi-GPU. To show the performance improvement, we compare both FP16 and INT8 version of the inference kernels 
with an efficient implementation provided by NVIDIA, called FasterTransformers (FT).
Regarding the model architectures, we explore different sizes, varying both the transformer model's inner dimension
(Hidden size) and number of layers. Table~\ref{t:model-configs} shows these detail of the model architectures.

To measure the inference performance, we use two metrics, inference-latency and throughput. 
Inference-latency is an important metric showing the quality of the use-experience, whereas
throughput shows the number of requests-per-second an inference system can process without
violating the service-level agreements (SLA). Even though inference throughput can improve by increasing
the batch-size, there is always the challenge of keeping the latency under the limit of satisfying the SLA. 
We show that DeepSpeed-Inference obtains both of these goals through the optimized kernels, reaching
a high memory-bandwidth and GPU core utilization during inference of different model structures.

\begin{table}[t!]
%\vskip -0.7em
\centering{
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Name & \# params & hidden dim & \# layers  & \# attention heads \\ \hline
    GPT-2 & 1.5B & 1.6K & 48 & 25 \\ \hline
    GPT-Neo & 2.7B & 2.5K & 32 & 20 \\ \hline
    GPT-J & 6B & 4K & 32 & 32 \\ \hline
    GPT-3-13B & 13B & 5K & 40 & 40 \\ \hline
    GPT-NeoX & 20B & 6K  & 44  & 64\\ \hline
    GPT-50B & 50B  & 8K & 62  & 64  \\ \hline
    GPT3-87B & 87B & 12K & 48 & 96\\ \hline
    GPT3-175B & 175B & 12K & 96 & 96\\ \hline
    MT-NLG 530B & 530B & 20K & 105 & 128\\ \hline
\end{tabular}
}
\caption{Model configurations used for the dense model inference performance evaluation.}
\label{t:model-configs}
\end{table}

\begin{figure*}[t]
\centering
\vskip -1.5em
\includegraphics[width=\textwidth, height=1.8in]{figures/kernels/single-gpu-inference1.pdf}
\caption{Single-GPU inference on different model sizes. We compare the latency and throughput of our 
FP16 and INT8 kernels with FT, using different batch sizes of 1, 8 and 16. 
achieves significant improvement both in terms of latency and inference throughput. }
\label{f:single-gpu-inference}
\end{figure*}

Figure~\ref{f:single-gpu-inference} shows how the inference-optimized kernels improve the inference latency
compared to a highly optimized baseline, as well as improving throughput while increasing the batch size from
1 up to 16. Comparing DS-FP16 performance with FT-fp16, we see between 20\% to 65\% speedups for different models
and batch-sizes. Furthermore, we boost the performance benefits even more by enabling INT8 kernels, getting between 35\%
and 2.5x speedups.
Diving deeper into these results, we see two trends when comparing DS and FT performance. On one side, we obtain larger improvement on
small batch size, where we have less computation and it requires high memory bandwidth to 
utilize the GPU cores. We address this by using the Deep-Fusion and the optimized GeMM scheduling techniques, reducing the inference-latency
between 50\% to 92\% which has a positive impact on the user-experience. On the other side, we reach higher throughput
for larger model sizes with larger batch size, that is due to the efficient kernel-fusion scheme employed for the large batch sizes, as well as
the highly optimized CUBLAS and CUTLASS GeMM kernels used for FP16 and INT8 data-types. This part of improvement enables the inference system to
process more requests while obtaining the SLA limit on fewer number of resources, significantly reducing the inference cost.

\begin{figure*}[t]
\centering
\vskip -1.5em
\includegraphics[width=\textwidth, height=1.8in]{figures/kernels/multi-gpu-inference2.pdf}
\caption{Multi-GPU inference on different model sizes. We use different model-parallelism, 2, 4, 8, and 16 for running inference
on different models, respectively.
Similar to Figure~\ref{f:single-gpu-inference} we see significant improvement comparing DeepSpeed with FT. }
\label{f:multi-gpu-inference}
\end{figure*}

To further evaluate our inference-optimized kernels, we consider large-scale models that require a multi-GPU inference solution. 
Figure~\ref{f:multi-gpu-inference} shows the multi-GPU inference performance of several model sizes between 20 to 175 billions parameters,
comparing DS-FP16 and DS-INT8 with the FT numbers. We use two 8-A100 DGX boxes for running these experiments. We also set the model-parallel (MP)
degree differently for each model size, 2, 4, 8, and 16-way MP for 20B, 50B, 87B, and 175B parameter sizes, respectively. 
In terms of performance improvements, we get optimization on both small and large batch sizes using either INT8 or FP16 kernels.
For batch size 1, since the model size is large enough, both FT and DS-FP16 achieve high memory-bandwidth utilization, 
and we only obtain minimal performance speedup (1-10\%). Whereas, by switching to INT8 kernel, we reduce the memory-bandwidth usage, 
providing more data to the tensor-cores INT8 units by utilizing similar bandwidth as the FP16 kernels. Thus, we can reduce the latency further (40\%-60\% speedups compared to FT) and 
improve the user-experience for the large-scale inference on these vast model sizes.
Regarding the larger batch sizes, we obtain 85\%-2.3x and 2.4x-2.9x speedups for the FP16 and INT8 versions of the kernels respectively.
Comparing the performance of INT8 and FP16 inference, we notice similar benefit as we increase the model-parallelism degree, due to the large
communication overhead caused by the all-reduce across GPUs. In the worst case of GPT-175, since we cross the node boundary and
this results in inter-node communication for the all-reduce, we see very small speedup compared to the rest. In Section~\ref{}, we show how the 
multi-dimensional parallelism, combining model-parallelism with pipeline parallelism, helps reduce this communication overhead.


==> inference-kernels.tex <==

\begin{figure*}[ht]
    \centering
    \vskip -1.5em
    \setlength{\abovecaptionskip}{-3pt}
    \resizebox{\textwidth}{!}{
    \subfigure[]{\includegraphics[width=0.35\textwidth]{figures/kernels/gemm-schedule12.png}} 
    \subfigure[]{\includegraphics[width=0.30\textwidth]{figures/kernels/gemm-schedule11.png}} 
    \subfigure[]{\includegraphics[width=0.35\textwidth]{figures/kernels/fusion.png}} 
    }
    \caption{ 
    (a) GEMM scheduling at different GPU architectural levels: threads-blocks, Warps and CUDA threads. Warps show different cooperative threads (32 threads), Lanes show the thread index at each Warp. 
    (b) GeMM Modification to support 2-dimensional partitioning of the weight matrix and new data-layout. (c) kernel-fusion. }
    % \minjia{Figure (b) needs to be adjusted to have a similar scale and font size as the other figures in this row.}
%    \minjia{Figure (b) looks a bit inproportional, e.g., the x-axis names occupy a huge portion of the figure. Can we adjust the x-axis such that some of the long texts are folded into two lines? This would give the figure a more proportional look. If it is hard to fold the text, another option to try is to switch the x and y axis so that the x-axis represents the speedups an the y-axis shows different configures. }
    \label{fig:gemm-schedule}
    \vspace{-10pt}
\end{figure*}

\section{Inference-Optimized Transformer Kernels}\label{sec:inference-kernels}

\begin{comment}
Inference of Transformer models comes with an interesting challenge. Even though, computationally, 
it is very similar to the forward pass of the training pipeline, however its workload varies dynamically 
based on the target application. The difference is due to the batch size (number of tokens) processed during the inference,
which can be very small (as small as 1 token) or very large (as in thousands of tokens). We consider different sets of 
optimizations to optimize the performance for either workloads. The small-batch inference is a memory-bound problem and
is very sensitive to the kernel-invocations and global memory data-transfer. Thus, we target the memory-bandwidth utilization
as the main optimization goal. On the other hand, the large-batch inference is a compute-bound problem that requires an 
efficient scheduling to maximize the GPU throughput. 
\end{comment}
In this section, we discuss the challenges, design, and optimizations for transformer kernels capable of achieve high-performance for both small and large batch size. 
%In this section, we go through the optimization techniques employed 
%to get the best performance for the different types of inference workloads.

\subsection{Inference Challenges on Different Batch Sizes}

\begin{comment}
GPU architecture is typically designed to provide high-throughput on large workload using many cores and thread-parallelism.
However, since there is not sufficient work dispatched by the small-batch inference, it is very difficult to get high-utilization from the GPU cores. 
This is due to the fact that such inference workload falls under the memory-bound region, which requires careful optimization scheme other than the 
normal GPGPU programming style that launches kernels with many blocks and threads to achieve the highest level of parallelism.
\end{comment}

As discussed in Sec.\ref{sec:introduction}, small batch performance is limited to by the memory bandwidth utilization in reading model weights. There are three main challenges to optimizing for memory bandwidth for small-batch sizes.
First, due to limited work at different kernels performing the operations of a transformer layer due to small batch size, 
inference performance suffers from the kernel-invocation overhead. Second, each kernel-invocation writes data to global memory which is read by GPU cores during the next kernel invocation, and this data-transfer between GPU cores and global memory adds an additional overhead. 
Finally, neither cuBLAS nor CUTLASS GeMM libraries are well tuned for extremely small batch sizes, and cannot achieve good memory-bandwidth utilization. 

Large-batch inference performance on the other-hand is limited by compute utilization, and while compute heavy operations like GEMM inside a transformer layer can achieve very good compute utilization using CUBLAS and CUTLASS libraries, the overall utilization can still be limited by the kernel launch overheads and data-transfers between GPU cores and global memory across different kernels other than GEMMs. 

\begin{comment}
that exist has besides the GeMM operations.
Thankfully, CUBLAS and CUTLASS libraries achieve good efficiency on the large-batch sizes, however, we still encounter
the low parallelism on several operators executed between the GeMMs. Similar to the small-batch inference, the inefficiency is
due to the kernel-invocation and the data-transfer happening between kernels.
\end{comment}


In order to address these challenges, we introduce two new techniques: i) Deep-Fusion to reduce kernel-invocation and data-movement overheads by fusing multiple kernels beyond element-wise operations, and ii) A custom GeMM kernel designed for improving the the memory bandwidth utilization when the batch size is relatively small while also allowing it to be fused using Deep-Fusion. We discuss these techniques in detail next.

%Regarding the large batch inference, we use the same Deep-Fusion technique as described in the previous section, with the difference that
%we use CUBLAS implementation for the GeMM operations and fuse the rest of operations. We take this fusion strategy due to two main reasons: first,
%CUBLAS library is very well-tuned for the large batch GeMM and achieve high throughput, and second, fusing GeMM with other operation is less efficient 
%since it adds more pressure on the register file or shared-memory for saving the intermediate results, restricting the number of threads
%the kernel can launch with. Except GeMM, the rest of the operations that have similar memory-access pattern, like layer-norm, bias-add, activation,
%and transposition are fused together through the Deep-Fusion scheme.

%DeepSpeed Inference uses Deep-Fusion and an optimized GeMM scheduling to build high-performance kernels for the different part of a Transformer layer.

\begin{figure*}[th!]
\centering
\includegraphics[width=0.9\textwidth]{figures/model-parallelism/pipeline_schedule.png}
\caption{A pipeline-parallel schedule for generating 4 sequences on 4 pipeline stages. {\color{blue} todo: clean up figure}} 
\label{fig:pipe-schedule}
\end{figure*}
\section{Inference-Optimized Dense Transformer Models on Many-GPU Systems}
\label{sec:many-gpu-dense}

\subsection{Deep-Fusion}
While operator fusion is a common technique used in deep learning to reduce kernel launch and data-movement overhead, it is limited primarily to element-wise operators  \cite{tensorflow_xla, chen2018tvm, ONNX_Runtime_developers_ONNX_Runtime_2018}. In contrast, transformer consists of operators like data layout transformations, reductions, and GeMMs which create data dependencies across thread blocks making them difficult to fuse. This is because on a GPU system, if a data produced by a thread-block is consumed by a different thread-block, a global memory synchronization is needed, and this synchronization is done by invoking a new kernel. 

To avoid the need for a global synchronization, deep-fusion tiles the computation space along dimensions of the iteration space which incur no cross-tile data-dependencies and executes them in parallel across different thread-blocks. The dimensions of the computation space which does contain data dependencies are not tiled, and instead processed by the same thread-block. 

After this tiling, two operators can be fused using deep-fusion if each tile of the second operator depends on exactly one output tile of the first operator. By performing fusion at tile granularity, Deep-Fusion can fuse not only element-wise operations but also reductions, data transpositions, and GEMMs as long as there are no cross-tile dependencies. For example, all micro-operations in a layer-norm \cite{layernorm} can be tiled along the token dimension, while the reduction dimensions are processed within a tile. This allows all the micro-operations inside a layernorm to be fused into a single kernel despite consisting of multiple reduction operations. Furthermore, the data produced by each tile is either kept in registers or in shared memory when possible to allow for data-reuse across operators without incurring global memory data-transfer overheads.

\begin{comment}
Unlike the existing fusion techniques that primarily fuse element-wise operations \cite{tensorflow_xla, chen2018tvm, ONNX_Runtime_developers_ONNX_Runtime_2018},
Deep-Fusion can fuse reductions, transpositions and matrix-multiplications in addition to element-wise operations.  
To do so, we identify 
Deep-Fusion brings a two-fold performance benefit, 
first it greatly reduces the number of kernel invocations therefore less kernel-call (CPU-to-GPU) overhead, 
second, it keeps the data persistent on the threads, either on registers or shared memory, 
which removes the data-movement overhead between GPU cores and global memory. 
Next, we evaluate the Deep-fusion's strategies taken for the small and large batch inference.

We take two main criteria when fusing operations together.
First, when choosing the operations for Deep-fusion, we keep the same pattern of accessing data for 
processing the sequence of operations that are fused together. This allows avoiding data-transfer between thread-blocks,
which otherwise results in communicating data between streaming multi-processors (SMs) and adds the overhead of synching 
them through global memory. Second, we consider fusing the operations that are between communication collectives such 
as all-reduce, letting the partial results merged across parallel GPUs before sending data to the next fused part of the transformer layer.
\end{comment}
%
\subsection{Custom GEMM for small batch size}

\begin{figure*}[ht]
    \centering
    \vskip -1.5em
    \setlength{\abovecaptionskip}{-3pt}
    \resizebox{\textwidth}{!}{
    \subfigure[]{\includegraphics[width=0.25\textwidth]{figures/kernels/gemm-schedule_combined.png}} 
    \subfigure[]{\includegraphics[width=0.25\textwidth]{figures/kernels/fusion.pdf}} 
    }
    \caption{ 
    (a) GeMM scheduling at different GPU architectural levels: threads-blocks, Warps and CUDA threads. Warps show different cooperative threads (32 threads), Lanes show the thread index at each Warp. 
    (b) kernel-fusion. }
    % \minjia{Figure (b) needs to be adjusted to have a similar scale and font size as the other figures in this row.}
%    \minjia{Figure (b) looks a bit inproportional, e.g., the x-axis names occupy a huge portion of the figure. Can we adjust the x-axis such that some of the long texts are folded into two lines? This would give the figure a more proportional look. If it is hard to fold the text, another option to try is to switch the x and y axis so that the x-axis represents the speedups an the y-axis shows different configures. }
    \label{fig:gemm-schedule}
    \vspace{-10pt}
\end{figure*}

%\begin{figure}[t!]
%\centering
%\vskip -1.5em
%\includegraphics[width=\columnwidth]{figures/kernels/gemm_schedule.pdf}
%\caption{GeMM scheduling at different GPU architectural levels: threads-blocks, Warps and CUDA threads. Warps show different cooperative threads (32 threads), Lanes show the thread index at each Warp. }
%\label{f:gemm-schedule}
%\vskip -1.5em
%\end{figure}
\begin{comment}
GeMM is the most important operation inside a transformer taking more than 60-70\% of the run-time. Therefore, unless this operation is fully optimized, our kernel fusion won’t be effective and cannot provide any performance speedup compared to using CUBLAS, non-fused implementation. Hence, we explore different approaches for scheduling the vector-matrix or skinny matrix-matrix multiplication. We found that the most promising schedule is based on Persistent-Threads (PT) programming style which takes into account the hardware architecture detail as well as the memory-access pattern in addition to keeping the data persistent on each thread. 
\end{comment}
Our custom GEMM implementation is designed to be fusable with deep-fusion while achieving maximum memory bandwidth utilization. Its design can be viewed in three parts:  tiling strategies, cooperative-group reduction, and data-layout transformation for better memory bandwidth utilization.

\paragraph{Tiling Strategies}
Figure~\ref{f:gemm-schedule} depicts our GeMM scheduling for a skinny matrix-matrix multiplication. We first tile the computation along the output dimension that allows us to implement GEMM using a single kernel by keeping the reduction within a tile. For small models, where the output dimension is too small to create enough parallel tiles to achieve good memory-bandwidth, we tile the input dimension as well, requiring GEMM to be implemented as two kernels to allow for reduction across tiles.

Figure~\ref{f:gemm-schedule} depicts our GeMM scheduling for a skinny matrix-matrix multiplication. We first tile the computation along the output dimension. With this 1D tiling, each warp can read a tile of columns with coalesced memory access to achieve high memory bandwidth utilization, and the reduction along the input dimension is computed within the tile with no cross-tile dependencies, allowing the GEMM to be implemented as a single kernel. 

\begin {comment}
and wraps across thread blocks can read different tile of columns for different rows.  and , as long as it is large enough to create enough parallel tiles to feed all the SMs, which is crucial to achieving high bandwidth.  

We partition the weight matrix in two directions: 1) column-wise across the threads of the first Warp of the thread-blocks (shown with the red lines), and 2) row-wise across the Warps at each block (shown with the blue lines). By assigning the columns to different blocks, we assure getting both coalesced access on weight matrix and good locality on the input matrix. Coalesced access is the result of consecutive memory access on the cooperative threads across different blocks, and input buffer is accessed in the same pattern across blocks which improves the cache locality. Moreover, we get high bandwidth from L1 cache as the concurrent 32 threads access the same cache line, by bringing 128 bytes of data at each Warp in the different SMs.   
\end{comment}
One caveat of this 1D tiling is that for small models it may under utilize SMs limiting the memory bandwidth utilization if the output size is not large enough to feed all the threads of the streaming multiprocessors (SMs) of the GPU. In this scenario, creating enough parallelism across SMs is more important than using a single kernel, therefore we add tiling along the input dimension.  Figure~\ref{f:gemm-schedule2} illustrates the 2-dimensional tiling in order to occupy more SMs than the one shown in Figure~\ref{f:gemm-schedule}. This way, we can use more thread parallelism to read the weight matrix and therefore boost the memory-bandwidth utilization. Since each group of blocks only process a part of the input dimension, we get partial GeMM computation at each section. To produce the final result, we use a separate kernel after the GeMM operation to reduce the results on different blocks.


\paragraph{Cooperative-Group Reduction}

With the above mentioned tiling strategy, each warp in a thread block is responsible for producing a partially reduced result for a tile of outputs and a final reduction is needed across all the warps within the thread block. One way to do this would be using a binary tree based approach where we perform pair-wise reduction by creating i) parallel warp pairs, ii) perform reduction between warp pairs, iii) write the results to shared memory, iv) perform a synchronization across warps and repeat from step i until the results are finally reduced at a single warp. However, the numerous warp level synchronizations, and shared memory read and writes create a performance bottleneck.

To address this, we first transpose the partially reduced results across warps using shared memory (see Figure~\ref{f:gemm-schedule}) such that threads in a warp hold different partially reduced element for the same output index that can then be fully reduced within the warp itself via cooperative-group collectives directly in registers, without requiring across warp synchronization in shared memory. After completion, the first thread of each warp holds the final result of a different element of the output matrix tile. Now, writing these results back directly to global memory would cause uncoalesced memory-access for the output matrix. Thus, we once again transpose data by the help of shared memory such that threads in a warp once again contains contiguous output elements which can be written back to memory with coalesced write to maximize memory bandwidth utilization.

\begin{comment}


to get the right pattern for writing data back to memory. This transposition also results in coalesced access to the output buffer across the different blocks. 


where intermediate reduction results are written in shared memory  , requiring a reduct

To perform the GeMM operation, a column segment is mapped to the all the Warps in a block. Each Warp computes the local GeMM over its own section of the weight matrix. We then use shared memory to transpose data in a way that each column’s data maps to one Warp as illustrated by the first transpose operation shown in Figure~\ref{f:gemm-schedule}. 
\end{comment}

\begin{figure}[t!]
\centering
\vskip -1.5em
\includegraphics[width=\columnwidth]{figures/kernels/gemm_schedule2.pdf}
\caption{Modification to the GeMM scheduling presented in Figure~\ref{f:gemm-schedule} to support 2-dimensional partitioning of the weight matrix. }
\label{f:gemm-schedule2}
\vskip -1.5em
\end{figure}

\paragraph{Data-layout Transformation for Better Memory Bandwidth Utilization}
In GPU architecture, each L1 cache-line is 128 bytes, and a coalesced memory access with a single fp32 element per thread in the warp can fully leverage each cache-line read. However, transformer models are trained in fp16, and a single fp16 element per thread in the warp can only use half the cache-line, resulting in wasted memory bandwidth. A naive approach to address this issue is to read multiple elements per thread along the output dimension. However, this increases the tilesize and reduces the number of parallel 1D tiles that can be scheduled, specially for small hidden sized models and hurt memory bandwidth utilization.

\begin{comment}
In addition to GeMM schedule, we consider a new data-layout for the weight-matrix in order to provide more data to each thread while reading the weight matrix. 
To this purpose, we consider the L1 cache size as the unit of memory data-read size for each Warp of a block. However, as we read data row-wise (along the output dimension),
we assign more outputs to each thread which can reduce the parallelism degree and hurt the GPU throughput for various model architectures. 
\end{comment}

To resolve this issue, we change the data-layout of the weight matrix during initialization, as depicted by Figure~\ref{f:gemmlayout}, to transpose each column partially such that each thread still computes the same number of elements along the output dimension but it reads multiple weight values ($M$) along the reduction dimension required to produce the output. $M$ can be set based on the memory hardware architecture and the data-type GeMM kernel is processing with. For instance, we set $M$ as 2 for half precision and 4 for the INT8 data types considering a 128-byte cache line.

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/kernels/gemmlayout.pdf}
\caption{GeMM layout transformation for increasing the L1-cache bandwith utilization}
\label{f:gemmlayout}
\end{figure}




\begin{figure}[t!]
\centering
\vskip -1.5em
\includegraphics[width=\columnwidth]{figures/kernels/fusion.pdf}
\caption{Transformer Layer with Megatron-style model-parallelism all-reduce components. The figure illustrates the parts of layer fused together with broken lines (width of line shows the fusion depth). }
\label{f:kernel-fusion}
\vskip -1.5em
\end{figure}

\subsection{Putting it together}

Small-batch Transformer Kernel: Figure~\ref{f:kernel-fusion} shows the different components of a transformer layer, and the operations which are considered for Deep-fusion 
in the small-batch inference case. As the figure shows, we fuse the operations inside a transformer layer at four main regions: 
1) the QKV GeMM and input layer-norm, 2) transposition plus attention, 3) post-attention layer-norm and intermediate GeMM, and 4) bias and residual addition. 
In order to support the fusion of GeMM with the rest of the operations in a single kernel for 3, 
we broadcast the input batch across the SMs and perform the same operations that comes before GeMM, 
so that there is no need of communicating data between SMs for adding the GeMM schedule. 
We observe that in spite of replicating the work across SMs, we still gain performance benefit 
compared to the non-replicated, non-fused kernel implementation for the very small batch sizes.


Large-batch Transfomer Kernel: Regarding the large batch inference, we slightly modify the fusion strategy by keeping the GeMM operations unfused, using CUBLAS implementation, and fusing the rest of operators as shown in Figure~\ref{f:kernel-fusion}. We make this modification to achieve higher throughput,
as the CUBLAS library is highly well-tuned for the big GeMM sizes. Furthermore, fusing GeMM operations with other operation is less efficient 
for large batch inference, since it adds more pressure on the register file or shared-memory for saving the intermediate results, 
restricting the number of threads the kernel can launch with and therefore reducing the parallelism degree and GPU utilization.

\begin{comment}
Deep-Fusion uses all the memory hierarchy levels available at the GPU architecture in order to distribute the work across threads and share data.
Thread registers are used for storing the the output results and for communicating data between operations. To communicate partial results across the reduction 
dimension and calculate final result, we employ each thread-block's shared-memory. 
Regarding the input, we read data in the thread registers when computing the reduction or element-wise operations and move the result to 
the shared-memory when fusing them the GeMM operation as it requires only a part of input at each computation step. 
\end{comment}




==> introduction.tex <==
\section{Introduction}\label{sec:introduction}
Transformer based models have been applied successfully across multiple domain (\cite{examples}) making it one of the most important model architecture in Deep Learning. A unique property of the transformer architecture is its scalability, that enables quality improvements by increasing the overall model size.  As a result, the size of the transformer based models have grown exponentially. Currently, the largest dense transformer model, MT-NLG 530B consists of a whopping half a trillion parameters. Furthermore, more recently sparse transformer models based on MoE architecture have demonstrated quality that can surpass dense models at the fraction of a training cost, but at much larger parameter count, resulting in models with multi-trillion parameters (/cite{}). 

{\color{blue} Rephrase this paragraph to make it more generic to transformers of all sizes, not just large ones}
At these enormous scales, these models demonstrate capabilities like X, Y, Z that seems to be straight out of science fiction. However, leveraging transformer models, big or small during inference is quite challenging. However, the massive parameter count that makes these models so capable, also makes it challenging to use for inference:

\subsection{Challenges}
{ \color{blue} TODO: We need to bring in throughout challenges here some how. We want to shift the entire Pareto frontier of latency vs throughput because both latency and cost are important even at small batch sizes. Right now the way its written, the importance of throughput is not showing up. Furthermore there are also cases where throughput at large batch size is important but is challenging to achieve due to memory challenges. Bringing in throughput challenge by itself is a bit complicated here because its deeply tied to memory challenge. On one hand, large models require many gpus and since tensor-parallelism gets worse latency at scale, we use pipeline parallelism which avoids latency degradation but requires different schedule for inference than for training to keep the pipeline full and scale throughput. On the other hand, large batch inference where throughput is critical requires large memory to fit the activations, and lack of memory for the activations presents challenges for achieving better throughput.}
\textbf{Latency Challenges} Using a transformer based model in production requires meeting stringent latency requirements. Meeting these latency constraints of a production workload requires a memory bandwidth centric optimization approach aimed at minimizing latency. Notice that inference latency of a model is lower bounded by  the time it takes to load all the model parameters from memory to registers. Therefore, the latency is inversely proportional to the achievable memory bandwidth. 

Creating a generic inference system for transformer workloads that is capable of maximizing the achievable memory bandwidth to minimize latency is challenging due to the heterogeneity in batch size, model size, and model characteristics:

\begin{itemize}
\item \textbf{Batch Size} During model training, the batch size to the model is relatively large compared to inference, and the performance is primarily limited by the peak compute of the device such as the tensor-cores of a GPU. During inference on the other-hand, the batch size is in most cases quite small for real-time inference, while it can also be moderately large for semi-real time inference and massive for offline inference scenarios. The compute focused model implementation designed to achieve high throughput during training is simply not usable during inference due to its stringent latency requirements, and require a more latency focused design based on the batch size of the workload. For example, small batch sizes require a solution aimed maximizing kernel fusion across a broad range of operators such as layer-norm, softmax and GEMM, to reduce kernel launch over-head and GPU-memory data movement to maximize memory bandwidth utilization. In contrast, large batch sizes require a solution geared primarily at optimizing GEMM computation to maximize compute utilization using CUBLAS or CUTLASS on tensor-cores. The heterogeneity in batch size therefore, makes it challenging to develop a homogeneous solutions for transformer inference. 

\item \textbf{Model Size} For a small transformer based models, the high bandwidth single GPU memory might be sufficient to meet the latency requirements, however, for larger models, even the peak memory bandwidth of a single device may not be sufficient to meet the latency constraints requiring aggregate memory bandwidth across multiple devices. Achieving high aggregate bandwidth across multiple devices require achieving high memory bandwidth per device as well as using optimal parallelism strategy for partitioning the model computation across devices that minimizes the communication overhead across devices. Unfortunately, there is not a single parallelism strategy that works for all models, and is highly dependent on model characteristics that we will discuss next.

\item \textbf{Model Characteristics}  Transformer based models can be broadly categorized as dense or sparse models based on Mixture-of-Experts (MoE), and the optimal parallelism strategy depends on the type of workload. For example, approaches like tensor-slicing, and pipeline parallelism work only for dense transformers, while expert-parallelism only work for sparse transformers. Transformer based MoE models contains both dense and sparse transformer components, requiring a combination of different parallelism techniques, to maximize the achievable memory bandwidth across devices.

Difference s in model characteristics not only require different parallelism strategies, but also a careful consideration of who theses parallelism strategies maps to the heterogeneous network characteristics of modern GPU cluster.=. Modern GPU clusters such as the NVIDIA DGX-2 super pod have have a heterogeneous network topology. Each node within a cluster consists of 1 to 16 NVIDIA GPUs connected via either PCI-e or the proprietary NVIDIA NVLINK/NVSwitch network that offer very high GPU-GPU bandwidth. Scaling out further, individual nodes are connected to each other via Infiniband network with a significantly lower GPU-GPU inter-node bandwidth compared to intra-node bandwidth. The parallelism strategy to scale the aggregate memory bandwidth across multiple GPU devices must account for the variation in network topology and charecteristics.
\end{itemize}

\textbf{Memory Challenges} A model with tens of billions of parameters is simply too large to fit in the memory of a single GPU device, and at hundreds of billions of parameters, it is too large to even fit in the aggregate GPU memory of a single node. For example, inferncing the MT-NLG 530B requires about 1TB of GPU memory just to fit the model for inference, requiring over three DGX-2 nodes consisting over two dozen of NVIDIA A100 40GB GPUs. Most data scientists simply do not have access to such GPU resources needed for inference of these massive models.

\subsection{DeepSpeed Inference}

In this paper, we present DeepSpeed Inference, comprehensive solution for transformer model inference designed to address the above mentioned challenges. DeepSpeed Inference consists of two components:

\subsubsection{GPU Inference System}

DeepSpeed GPU Inference System, is a GPU only solution, designed to minimize latency while maximizing throughput for both dense and sparse transformer models. It can achieve state-of-art latency and throughput for transformer models of all sizes, and is capable of running on a single GPU or scaling to hundreds of GPUs to inference a multi-trillion parameter model. The GPU Inference solution is a three-layered system architecture designed to address the latency challenges of transformer model inference:

i) Single GPU transformer kernels: At the heart of our solution are the single GPU transformer kernels designed to maximize bandwidth utilization to minimize latency, while maximizing throughput at both small and large batch sizes to address the heterogeneity in batch size. These kernels form core building blocks of DeepSpeed Transformer Inference, and rest of the DeepSpeed Transformer Inference is built on top of it.

ii) Many-GPU dense transformer layer: This layer is built on top of single gpu transformer kernels and is capable of leveraging tensor-slicing to leverage aggregate memory bandwidth across multiple GPUs within a node, and pipeline parallelism to accommodate massive model sizes with minimal impact to latency, while achieving near linear throughput scaling across nodes. It builds new pipeline schedules to reduce pipeline stalls for inference to minimize overall latency, and memory offloading with communication optimizations strategies to enable larger batch sizes for higher throughput.  

iii) Massive-GPU scale sparse model layer: This layer is built on top of the previous two layers for sparse MoE models consisting of both dense transformer blocks and sparse MoE layers. It is designed to scale a sparse MoE model inference  to achieve an unprecedented level of aggregate memory bandwidth across hundred of GPUs to reduce inference latency of even the most massive sparse models. To do so we leverage expert-parallelism for sparse layers and data-parallelism along with tensor-slicing from the dense layers, while developing novel and holistic communication optimizations that are essential to reduce communication overhead needed to enable inference at this scale. In addition, we develop MoE specific kernels that reduces the complexity of MoE gating functions from cubic to quadratic to avoid compute bottlenecks that limit achievable single GPU memory bandwidth so that we make the most of each GPU.  

By taking this layered approach, where each layer address a unique aspect of the latency challenge: batch size, scaling dense models, and scaling sparse models, but are compatible and built on top of each other, we create a comprehensive system capable of achieving state-of-art latency and throughput at all scales for both dense and sparse transformer models despite the heterogeneity in batch size, model scale and model characteristics.

\subsubsection{ZeRO-Inference System}

DeepSpeed ZeRO-Inference System, is a heterogeneous GPU+CPU+NVMe based solution for specifically addressing the memory challenge by enabling massive model inference with minimal GPU resources. For applications that are not latency critical, ZeRO-Inference allows large batch inference of models with hundreds of billions of parameters on a single or multiple GPUs with high efficiency, as long as there is enough CPU or NVMe storage to store the model parameters. {\color{blue} elaborate this a bit more}

The main contributions of this paper are as follows:
\begin{itemize}
    \item Single GPU transformer kernels for inference and its evaluation
    \item Many-GPU dense transformer and its evaluation
    \item Massive-GPU scale sparse model inference and its evaluation
    \item ZeRO-Inference System and its evaluation
\end{itemize}

In the rest of the paper we first discuss related works, followed by sections discussing i) Single GPU transformer kernels, ii) Many-GPU dense transformer inference, iii) Massive-GPU scale sparse model inference, iv) ZeRO-Inference System, and v) Evaluation Section ...

\begin{comment}

Thi The many-gpu sparse transformer layer is built on top of the dense layer. It reuses the tensor-slicing based dense transformer layers build on top of our single GPU kernels for the dense components of the model, while adding expert-parallelism, data-parallelism and a multitude of communication optimization strategies to scale MoE based models to hundreds of GPUs to achieve an unprecedented levels of memory bandwidth for inferencing. In addition, the sparse transformer layer also consists of high performance kernels that are specific to 

\subsubsection{ZeRO-Inference System}
At the next layer  Our solution is based on a fundamental observation that a comprehensive solution to the challenges above requires independent solutions to three key problems: i) batch size, ii) model architecture, and iii) model scale. 

the primary source of heterogeneity in the problem space is the widely varying scale of transformer models, however,     

DeepSpeed Transformer Inference is capable of: i) Achieving state-of-art latency for both dense and sparse transformer models of all sizes, ii) Achieve state-of-art throughput for a given latency budget, iii)  for transformer model inference of all sizes capable of addressing all of the above challenges.  DeepSpeed-Inference consists of four high level components: 
\begin{itemize}
\item Single-GPU dense transformer kernels targeted at minimizing latency and maximizing throughput based on batch size.
\item Many-GPU dense inference system for latency constrained dense model inference: Short description of what it is
\item Many-GPU sparse inference system for latency constrained sparse model inference: Short description of what it is
\item ZeRO-Inference system to enable massive model inference on GPU memory constrained systems: SHort description of what it is
\end{itemize}


surpassing the state-of-art in multiple scenarios:
\begin{itemize}
    \item {GPU memory constrained system} It enables unprecedented model scale for inference on GPU memory constrained system by leveraging NVMe and CPU memory. More specific results: 
    \item {Single GPU dense transformer} It achieves x lower latency and y higher throughput than state-of-art from single GPU inference on model size up to M
    \item {Multi-GPU dense transformer} It can scaling to X GPUs, achieving latency reduction of Nx and thoughput increase of Zx compared to state-of-art for models up to Z billion parameters
    \item {Multi-GPU sparse transformer} It can inference an unprecedented multi-trillion parameters model in Xms scaling to an incredible N GPUs. This is the first system capable of scaling to Yx of GPUs for inference 
\end{itemize}

Optimizing for inference latency requires maximizing memory bandwidth utilization instead of maximizing compute utilization. . Therefore, it is crucial to maximize the achievable memory bandwidth for inference. Doing so is challenging because ... 

\begin{itemize}



\item A highly optimized inference implementation that can achieve a significant portion of the GPU memory bandwidth is not sufficient to meet latency requirements of large models. Note that modern GPUs like the NVIDIA V100 or the A100 have extremely high memory bandwidth of up to 2 TB/s, and with bandwidth centric optimizations, this bandwidth is sufficient to meet latency requirements for small models. However, for models with billions of parameters this is no longer the case. For example, a 40B parameter model running on a NVIDIA A100 80GB GPU with 2TB/s of memory bandwidth will have a minimum latency of 40 ms (40 *2/2000 sec), while the production latency requirements can be in the low 10 ms for tasks such as next token generation. 

\item Reducing the latency further to meet these stringent latencies require leveraging aggregate memory bandwidth across multiple GPU devices in parallel while minimizing the communication overhead. 

\item \textbf{Cost Challenges} Inference solutions  must not only meet the latency requirements but also maximize throughput 

 Doing so requires developing workload specific parallelization strategies that partitions the model computation across GPUs while while minimizing the communication overhead across devices otherwise degrade the latency.



The training system designed for training efficiency is simply not optimized inference latency,  , and leveraging massive models for these workloads requires meeting these requirements.  For example, a sentence completion feature should have no more than a few hundred millisecond latency so that it appears to be working in real time to enable users to productively leverage the feature without waiting for the suggestions to appear. There are other scenarios where the latency requirements can be as low as a few milliseconds.

The inference latency of a model is lower bounded by the time it takes to load the model parameters. This time is given by the ratio between the model size and achievable memory bandwidth. Note that for a model like, MT-NLG 530B, with a model size of over 1TB (in fp16), even the peak GPU memory bandwidth of 1.5TB/s would result in a latency of 700 ms, which is simply not acceptable for many production workloads. 
 
\item \textbf {Cost or Throughput Requirements} The cost of an inferencing solution is inversely proportional to the achievable throughput. While latency requirements dictates the response time, the cost or throughput requirements dictates the total number of requests that must be serviced using the a fixed number of GPU resources per unit time, without violating the latency requirements.

For example, for a latency requirement of 100ms, an inferencing solution that can process a thousands requests per second using a single GPU, while maintaining per request latency under 100ms is twice as expensive as a solution that can process two thousand request per second using a single GPU while also maintaining per request latency under 100ms. 


\end{itemize}


Even if the memory and latency requirements can be met, a model that requires significant resources for ineferncing is not practically viable from a cost standpoint. For example, it maybe possible to inference a GPT-3 sized model with a per token generation latency of 50ms using 16 NVIDIA A100 GPUs, however, if .....
On one hand, many data scientist do not have access to such resources to even try out models at this scale, while on the other hand, even when they do, partitioning and paralleling the model inference across dozens of GPUs is complex, and beyond the skill set of most data scientist.
\begin{itemize}
\item \textbf{Memory Challenge} : A model with tens of billions of parameters is simply too large to fit in the memory of a single GPU device such as NVIDIA A100 40GB, and at hundreds of billions of parameters, it is too large to even fit in the aggregate GPU memory of a single node such as the DGX-2 box which contains 8 such GPUs. A model like MT-NLG 530B would require aggregate GPU memory across dozens of GPUs. On one hand, many data scientist do not have access to such resources to even try out models at this scale, while on the other hand, even when they do, partitioning and paralleling the model inference across dozens of GPUs is complex, and beyond the skill set of most data scientist.

\item \textbf{Latency Challenge} Production workloads have strict latency requirements, and leveraging massive models for these workloads requires meeting these requirements. For example, a sentence completion feature should have no more than a few hundred millisecond latency so that it appears to be working in real time to enable users to productively leverage the feature without waiting for the suggestions to appear. There are other scenarios where the latency requirements can be as low as a few milliseconds.

The inference latency of a model is lower bounded by the time it takes to load the model parameters. This time is given by the ratio between the model size and achievable memory bandwidth. Note that for a model like, MT-NLG 530B, with a model size of over 1TB (in fp16), even the peak GPU memory bandwidth of 1.5TB/s would result in a latency of 700 ms, which is simply not acceptable for many production workloads. 

Reducing latency further requires leveraging the aggregate memory bandwidth across multiple GPU devices in parallel. 
iii) Cost Challenge
\end{itemize}



To fully leverage the quality of these massive transformer based model

It is clear that the quality of transformer based models, both dense and sparse, improves with model size, and hence there has been significant investment in training these massive models. However, the same techniques used for training these massive models do apply directly to inferncing them 
The size of transformer based models on both dense and sparse front are growing exponentially and inferencing them is becoming a major challenge. Exploitation of the capabilities of these large models lies in the ability to inference them at reasonable latencies, throughput and under resource budgets
	Memory Challenge
		Does not fit in a single GPU
		Does not fit in single node
	
	Latency and Throughput Challenge
		Larger the model, 
			higher bandwidth we need to achieve low latency
			Higher compute we need to achieve high throughput
		
		Latency Challenge
			Need to leverage the bandwidth across a large number of devices
				High bandwidth per device
		
		Throughput Challenge
			Need to leverage compute across a large number of devices
			High Throughput per device
			Back to memory challenge
			Scalable to a large number of GPUs without the communication becoming a bottleneck
			
			
		Heterogeneity 
			in hardware architecture
				GPUs connected with NVLINKs, connected InfiniBand
			Heterogeneity in mode architecture
			Requires Heterogeneity in parallelism and communication
		
		Solutions to training does not apply directly to inference
			Training latency is irrelevant, we only care about throughput
			We do not care about bandwidth utilization, instead about compute
			Batch size is large

The two fold goal is to tackle these challenges by developing techniques that enables inferencing transformer based models ranging from a few hundred million parameters, to hundreds of billions and even trillions of parameters with the following consideration:
	System Design for Extreme Scale and Performance to minimize latency and maximize thoughput
			Single GPU
			Within Node
			Across Nodes
	
	Democratization of large model inference
		Transcend memory limitations enabling large model inference on limited resources to enable non latency and throughput critical areas . Impossible-> Possible
	

DeepSpeed Inference
	Extreme Performance and Scale
		Optimizations at all scales, starting at single GPU and building upon it to scale to a node to hundreds of GPUs
		
		Single GPU Transformer (Reza)
			Limitations of implementation for training
			Maximizing bandwidth and compute utilization
			Shifting implementation based on workload characteristics
				Memory latency vs Bandwidth
		
		Inference Optimized 3D-Parallelism (Du, Shaden, Elton)
			Did we do anything special for tensor-slicing?
			Going beyond tensor-slicing
				Limitation of implementation for training on inference
				Inference challenges of 3D-Paralleism
				Our solutions
			
		Inference Optimized MoE (Ammar)
			Bring from the blog and our current paper
	
	Democratization of large model inference (Tunji, Cheng, Jeff)
		Inference Optimized ZeRO-Infinity
		
\end{comment}

==> introduction2.tex <==
\section{Introduction}
Transformer based models are capable of solving challenging problems across multiple domain (\cite{examples}) making it one of the most important model architecture in Deep Learning. Depending on type and complexity of the problem, the size and architecture of the transformer model can greatly vary, ranging from a few hundred million to hundreds of billions or even trillions of parameters in size, and built using dense \cite{dense-transformers} or sparse \cite{moe} components.
\begin{comment}
A unique property of the transformer architecture is its scalability, that enables capability and quality improvements by increasing the overall model size. As a result, transformer based models of varying sizes are used to solve problems with varying complexity, with models ranging from a few hundred million parameter (Bert \cite{bert}) to hundreds of billions of parameters (MT-NLG 530B \cite{mt-nlg}). Training dense transformer models at the larger end of this spectrum is extremely expensive, and as a result, sparse transformer models \cite{moe} have appeared recently that reduces the training cost, but are also much larger than their dense counter-parts consisting of trillions of parameters.

While these varied transformer based models can demonstrate capabilities like X, Y, Z that seems to be straight out of science fiction, using them in practice is not easy. 
\end{comment}
This heterogeneity in size and architecture of transformer models make it difficult to create effective system to inference them in practice, specially while meeting the stringent latency and cost requirements in production, or in the absence of massive amount of GPU resources required to just fit some of these models. More specifically, there are three main challenges towards using transformer based models for inference:

\textbf{Latency Challenges} Using a transformer based model in production requires meeting stringent latency requirements. As a result, the batch sizes used in production are generally small. For small batch sizes, inference latency of a model is lower bounded by the time it takes to load all the model parameters from memory to registers. Meeting the latency requirements of a transformer model inference is equivalent to achieving adequate memory bandwidth. However, creating a generic system capable of maximizing the achievable memory bandwidth to minimize latency is challenging due to the heterogeneity in the workload and hardware:

\begin{itemize}
\item \textbf{Small Batch Sizes} Maximizing achieved memory bandwidth at small batch sizes requires i) reading memory at near peak memory bandwidth for linear layers which consists of majority of the model weights, ii) achieving enough compute throughput to overlap compute with reading weight parameters and iii) minimizing kernel launch and data movement overhead of other operators like layernorm, softmax, etc. At extremely small batch sizes i) ,and iii) are critical, while for small batch sizes, i), ii) and iii) are all equally important, requiring different set of optimization depending on the actual batch size, even for small batch sizes. Furthermore, optimized kernels designed for training transformer models do not apply here as they only focus on maximizing compute utilization at very large batch sizes.


\item \textbf{Model Size} For a small transformer based models, the high bandwidth single GPU memory might be sufficient to meet the latency requirements, however, for larger models, even the peak memory bandwidth of a single device may not be sufficient to meet the latency constraints requiring aggregate memory bandwidth across multiple devices. Achieving high aggregate bandwidth across multiple devices require achieving high memory bandwidth per device as well as using optimal parallelism strategy for partitioning the model computation across devices that minimizes the communication overhead across devices. Unfortunately, there is not a single parallelism strategy that works for all models, and is highly dependent on model characteristics that we will discuss next.

\item \textbf{Model and Hardware Characteristics}  Transformer based models can be broadly categorized as dense or sparse models based on Mixture-of-Experts (MoE), and the optimal parallelism strategy depends on the type of workload. For example, approaches like tensor-slicing, and pipeline parallelism work only for dense transformers, while expert-parallelism only work for sparse transformers. Transformer based MoE models contains both dense and sparse transformer components, requiring a combination of different parallelism techniques, to maximize the achievable memory bandwidth across devices. Furthermore, modern clusters have heterogeneous network topology (eg. intra-node nvlink/nvswitch and inter-node infiniband). The parallelism strategy to scale the aggregate memory bandwidth across multiple GPU devices must also account for the variation in network topology and characteristics. 

\begin{comment}
Differences in model characteristics not only require different parallelism strategies, but also a careful consideration of who theses parallelism strategies maps to the heterogeneous network characteristics of modern GPU cluster.=. Modern GPU clusters such as the NVIDIA DGX-2 super pod have have a heterogeneous network topology. Each node within a cluster consists of 1 to 16 NVIDIA GPUs connected via either PCI-e or the proprietary NVIDIA NVLINK/NVSwitch network that offer very high GPU-GPU bandwidth. Scaling out further, individual nodes are connected to each other via Infiniband network with a significantly lower GPU-GPU inter-node bandwidth compared to intra-node bandwidth. 
\end{comment}
\end{itemize}

\textbf{Throughput Challenges}: In addition to meeting latency, production workloads also have throughput targets to meet cost budget. At small batch sizes, where the workload is still memory bandwidth bound, the latency of the workload does not increase as long as the computation is entirely overlapped with model weight reads. Therefore, maximizing throughput while meeting the latency SLA requires not only maximizing the memory bandwidth utilization, but also overlapping compute with the model weight reads, and achieving high compute efficiency at small batch sizes to maximize the batch size whose compute can be overlapped with reading the model weights. Inference kernels must therefore achieve high memory bandwidth utilization and high compute utilization at small batch sizes, whereas training kernels simply need to achieve high compute utilization at much larger batch sizes. This makes developing inference kernels quite challenging.

In addition, inference workloads can also significantly differ from training workloads in terms of data flow and computation dependencies, requiring novel solutions to achieve high throughput even at large batch sizes for non-latency critical applications. For example, generative transformer models have dependencies between each generated token and the next token, that does not exist during training. As a result, they have much higher memory requirement during inference to keep track of previously generated states. Furthermore, for large models that use pipeline parallelism, this dependency across generated tokens requires new pipeline schedules to keep all devices busy compared to training scenarios.

\textbf{Accessibility Challenges}: A model with tens of billions of parameters is simply too large to fit in the memory of a single GPU device, and at hundreds of billions of parameters, it is too large to even fit in the aggregate GPU memory of a single node. For example, inferncing the MT-NLG 530B requires about 1TB of GPU memory just to fit the model for inference, requiring over three DGX-2 nodes consisting over two dozen of NVIDIA A100 40GB GPUs. Most data scientists simply do not have access to such GPU resources needed for inference of these massive models.

\subsection{DeepSpeed Inference}

In this paper, we present DeepSpeed Inference, comprehensive solution for transformer model inference designed to address the above mentioned challenges. DeepSpeed Inference consists of two components:

\subsubsection{GPU Inference System}

DeepSpeed GPU Inference System, is a GPU only solution, designed to minimize latency while maximizing throughput for both dense and sparse transformer models. It can achieve state-of-art latency and throughput for transformer models of all sizes, and is capable of running on a single GPU or scaling to hundreds of GPUs to inference a multi-trillion parameter model. The GPU Inference solution is a three-layered system architecture designed to address the latency challenges of transformer model inference:

i) Single GPU transformer kernels: At the heart of our solution are the single GPU transformer kernels designed to maximize bandwidth utilization to minimize latency, while maximizing throughput at both small and large batch sizes to address the heterogeneity in batch size. These kernels form core building blocks of DeepSpeed Transformer Inference, and rest of the DeepSpeed Transformer Inference is built on top of it.

ii) Many-GPU dense transformer layer: This layer is built on top of single gpu transformer kernels and is capable of leveraging tensor-slicing to leverage aggregate memory bandwidth across multiple GPUs within a node, and pipeline parallelism to accommodate massive model sizes with minimal impact to latency, while achieving near linear throughput scaling across nodes. It builds new pipeline schedules to reduce pipeline stalls for inference to minimize overall latency, and memory offloading with communication optimizations strategies to enable larger batch sizes for higher throughput.  

iii) Massive-GPU scale sparse model layer: This layer is built on top of the previous two layers for sparse MoE models consisting of both dense transformer blocks and sparse MoE layers. It is designed to scale a sparse MoE model inference  to achieve an unprecedented level of aggregate memory bandwidth across hundred of GPUs to reduce inference latency of even the most massive sparse models. To do so we leverage expert-parallelism for sparse layers and data-parallelism along with tensor-slicing from the dense layers, while developing novel and holistic communication optimizations that are essential to reduce communication overhead needed to enable inference at this scale. In addition, we develop MoE specific kernels that reduces the complexity of MoE gating functions from cubic to quadratic to avoid compute bottlenecks that limit achievable single GPU memory bandwidth so that we make the most of each GPU.  

By taking this layered approach, where each layer address a unique aspect of the latency challenge: batch size, scaling dense models, and scaling sparse models, but are compatible and built on top of each other, we create a comprehensive system capable of achieving state-of-art latency and throughput at all scales for both dense and sparse transformer models despite the heterogeneity in batch size, model scale and model characteristics.

\subsubsection{ZeRO-Inference System}
DeepSpeed ZeRO-Inference System, is a heterogeneous GPU+CPU+NVMe based solution for specifically addressing the memory challenge by enabling massive model inference with minimal GPU resources. For applications that are not latency critical, ZeRO-Inference allows large batch inference of models with hundreds of billions of parameters on a single or multiple GPUs with high efficiency, as long as there is enough CPU or NVMe storage to store the model parameters. {\color{blue} elaborate this a bit more}

The main contributions of this \name are as follows:
\begin{itemize}
    \item Single GPU transformer kernels for minimizing latency and maximizing throughput via memory-bandwidth-centric fusion schedules and GEMM kernels
    \item Many-GPU dense transformer inference system that combines tensor-parallelism to minimize latency with new inference optimized pipeline parallelism schedules and memory optimizations strategy to maximize throughput.
    \item An massive-GPU scale sparse model inference that combines: i) expert,data and tensor-parallelism, ii) novel communication optimization strategies and iii) sparse model specific kernels optimizations achieving real-time latency at trillion parameter model scale
    \item ZeRO-Inference that leverages CPU, NVMe and GPU memory along with GPU compute to make massive model inference accessible with limited resources.  
    \item An extensive evaluation of all the above mentioned components: a) Up to X lower latency and Y higher throughput for dense transformer models ranging from 300M to 500B parameters on up to 35 NVIDIA A100 GPUs compared to the state-of-art FasterTransformer library from NVIDIA \cite{faster-transformer} for transformer model inference. b) Up to Nx lower latency than state-of-art sparse transformer implementations for model sizes ranging from 52B to 2Trillion. \name can inference a trillion parameter sparse model under Z ms with aggregate bandwidth of over Y TB/s by scaling to an unprecedented N GPUs for inference. For reference, the fastest dense transformer implementation with Y parameters takes Z ms while consisting of Nx lower number of parameters. c) \name can inference half a trillion parameter model requiring 1TB of memory on a single GPU with mere 40 GB of memory by leveraging NVMe or CPU memory with a throughput an excellent compute efficiency of X percent (X TFlops). For models large models that fit in GPU memory, \name can achieve up to X percent higher throughput by using ZeRO-Inference to enable large batch sizes. 
\end{itemize}

Concluding remark.. 

In the rest of the paper we first discuss related works, followed by sections discussing i) Single GPU transformer kernels, ii) Many-GPU dense transformer inference, iii) Massive-GPU scale sparse model inference, iv) ZeRO-Inference System, and v) Evaluation Section.

\begin{comment}

Thi The many-gpu sparse transformer layer is built on top of the dense layer. It reuses the tensor-slicing based dense transformer layers build on top of our single GPU kernels for the dense components of the model, while adding expert-parallelism, data-parallelism and a multitude of communication optimization strategies to scale MoE based models to hundreds of GPUs to achieve an unprecedented levels of memory bandwidth for inferencing. In addition, the sparse transformer layer also consists of high performance kernels that are specific to 

\subsubsection{ZeRO-Inference System}
At the next layer  Our solution is based on a fundamental observation that a comprehensive solution to the challenges above requires independent solutions to three key problems: i) batch size, ii) model architecture, and iii) model scale. 

the primary source of heterogeneity in the problem space is the widely varying scale of transformer models, however,     

DeepSpeed Transformer Inference is capable of: i) Achieving state-of-art latency for both dense and sparse transformer models of all sizes, ii) Achieve state-of-art throughput for a given latency budget, iii)  for transformer model inference of all sizes capable of addressing all of the above challenges.  DeepSpeed-Inference consists of four high level components: 
\begin{itemize}
\item Single-GPU dense transformer kernels targeted at minimizing latency and maximizing throughput based on batch size.
\item Many-GPU dense inference system for latency constrained dense model inference: Short description of what it is
\item Many-GPU sparse inference system for latency constrained sparse model inference: Short description of what it is
\item ZeRO-Inference system to enable massive model inference on GPU memory constrained systems: SHort description of what it is
\end{itemize}


surpassing the state-of-art in multiple scenarios:
\begin{itemize}
    \item {GPU memory constrained system} It enables unprecedented model scale for inference on GPU memory constrained system by leveraging NVMe and CPU memory. More specific results: 
    \item {Single GPU dense transformer} It achieves x lower latency and y higher throughput than state-of-art from single GPU inference on model size up to M
    \item {Multi-GPU dense transformer} It can scaling to X GPUs, achieving latency reduction of Nx and thoughput increase of Zx compared to state-of-art for models up to Z billion parameters
    \item {Multi-GPU sparse transformer} It can inference an unprecedented multi-trillion parameters model in Xms scaling to an incredible N GPUs. This is the first system capable of scaling to Yx of GPUs for inference 
\end{itemize}

Optimizing for inference latency requires maximizing memory bandwidth utilization instead of maximizing compute utilization. . Therefore, it is crucial to maximize the achievable memory bandwidth for inference. Doing so is challenging because ... 

\begin{itemize}



\item A highly optimized inference implementation that can achieve a significant portion of the GPU memory bandwidth is not sufficient to meet latency requirements of large models. Note that modern GPUs like the NVIDIA V100 or the A100 have extremely high memory bandwidth of up to 2 TB/s, and with bandwidth centric optimizations, this bandwidth is sufficient to meet latency requirements for small models. However, for models with billions of parameters this is no longer the case. For example, a 40B parameter model running on a NVIDIA A100 80GB GPU with 2TB/s of memory bandwidth will have a minimum latency of 40 ms (40 *2/2000 sec), while the production latency requirements can be in the low 10 ms for tasks such as next token generation. 

\item Reducing the latency further to meet these stringent latencies require leveraging aggregate memory bandwidth across multiple GPU devices in parallel while minimizing the communication overhead. 

\item \textbf{Cost Challenges} Inference solutions  must not only meet the latency requirements but also maximize throughput 

 Doing so requires developing workload specific parallelization strategies that partitions the model computation across GPUs while while minimizing the communication overhead across devices otherwise degrade the latency.



The training system designed for training efficiency is simply not optimized inference latency,  , and leveraging massive models for these workloads requires meeting these requirements.  For example, a sentence completion feature should have no more than a few hundred millisecond latency so that it appears to be working in real time to enable users to productively leverage the feature without waiting for the suggestions to appear. There are other scenarios where the latency requirements can be as low as a few milliseconds.

The inference latency of a model is lower bounded by the time it takes to load the model parameters. This time is given by the ratio between the model size and achievable memory bandwidth. Note that for a model like, MT-NLG 530B, with a model size of over 1TB (in fp16), even the peak GPU memory bandwidth of 1.5TB/s would result in a latency of 700 ms, which is simply not acceptable for many production workloads. 
 
\item \textbf {Cost or Throughput Requirements} The cost of an inferencing solution is inversely proportional to the achievable throughput. While latency requirements dictates the response time, the cost or throughput requirements dictates the total number of requests that must be serviced using the a fixed number of GPU resources per unit time, without violating the latency requirements.

For example, for a latency requirement of 100ms, an inferencing solution that can process a thousands requests per second using a single GPU, while maintaining per request latency under 100ms is twice as expensive as a solution that can process two thousand request per second using a single GPU while also maintaining per request latency under 100ms. 


\end{itemize}


Even if the memory and latency requirements can be met, a model that requires significant resources for ineferncing is not practically viable from a cost standpoint. For example, it maybe possible to inference a GPT-3 sized model with a per token generation latency of 50ms using 16 NVIDIA A100 GPUs, however, if .....
On one hand, many data scientist do not have access to such resources to even try out models at this scale, while on the other hand, even when they do, partitioning and paralleling the model inference across dozens of GPUs is complex, and beyond the skill set of most data scientist.
\begin{itemize}
\item \textbf{Memory Challenge} : A model with tens of billions of parameters is simply too large to fit in the memory of a single GPU device such as NVIDIA A100 40GB, and at hundreds of billions of parameters, it is too large to even fit in the aggregate GPU memory of a single node such as the DGX-2 box which contains 8 such GPUs. A model like MT-NLG 530B would require aggregate GPU memory across dozens of GPUs. On one hand, many data scientist do not have access to such resources to even try out models at this scale, while on the other hand, even when they do, partitioning and paralleling the model inference across dozens of GPUs is complex, and beyond the skill set of most data scientist.

\item \textbf{Latency Challenge} Production workloads have strict latency requirements, and leveraging massive models for these workloads requires meeting these requirements. For example, a sentence completion feature should have no more than a few hundred millisecond latency so that it appears to be working in real time to enable users to productively leverage the feature without waiting for the suggestions to appear. There are other scenarios where the latency requirements can be as low as a few milliseconds.

The inference latency of a model is lower bounded by the time it takes to load the model parameters. This time is given by the ratio between the model size and achievable memory bandwidth. Note that for a model like, MT-NLG 530B, with a model size of over 1TB (in fp16), even the peak GPU memory bandwidth of 1.5TB/s would result in a latency of 700 ms, which is simply not acceptable for many production workloads. 

Reducing latency further requires leveraging the aggregate memory bandwidth across multiple GPU devices in parallel. 
iii) Cost Challenge
\end{itemize}



To fully leverage the quality of these massive transformer based model

It is clear that the quality of transformer based models, both dense and sparse, improves with model size, and hence there has been significant investment in training these massive models. However, the same techniques used for training these massive models do apply directly to inferncing them 
The size of transformer based models on both dense and sparse front are growing exponentially and inferencing them is becoming a major challenge. Exploitation of the capabilities of these large models lies in the ability to inference them at reasonable latencies, throughput and under resource budgets
	Memory Challenge
		Does not fit in a single GPU
		Does not fit in single node
	
	Latency and Throughput Challenge
		Larger the model, 
			higher bandwidth we need to achieve low latency
			Higher compute we need to achieve high throughput
		
		Latency Challenge
			Need to leverage the bandwidth across a large number of devices
				High bandwidth per device
		
		Throughput Challenge
			Need to leverage compute across a large number of devices
			High Throughput per device
			Back to memory challenge
			Scalable to a large number of GPUs without the communication becoming a bottleneck
			
			
		Heterogeneity 
			in hardware architecture
				GPUs connected with NVLINKs, connected InfiniBand
			Heterogeneity in mode architecture
			Requires Heterogeneity in parallelism and communication
		
		Solutions to training does not apply directly to inference
			Training latency is irrelevant, we only care about throughput
			We do not care about bandwidth utilization, instead about compute
			Batch size is large

The two fold goal is to tackle these challenges by developing techniques that enables inferencing transformer based models ranging from a few hundred million parameters, to hundreds of billions and even trillions of parameters with the following consideration:
	System Design for Extreme Scale and Performance to minimize latency and maximize thoughput
			Single GPU
			Within Node
			Across Nodes
	
	Democratization of large model inference
		Transcend memory limitations enabling large model inference on limited resources to enable non latency and throughput critical areas . Impossible-> Possible
	

DeepSpeed Inference
	Extreme Performance and Scale
		Optimizations at all scales, starting at single GPU and building upon it to scale to a node to hundreds of GPUs
		
		Single GPU Transformer (Reza)
			Limitations of implementation for training
			Maximizing bandwidth and compute utilization
			Shifting implementation based on workload characteristics
				Memory latency vs Bandwidth
		
		Inference Optimized 3D-Parallelism (Du, Shaden, Elton)
			Did we do anything special for tensor-slicing?
			Going beyond tensor-slicing
				Limitation of implementation for training on inference
				Inference challenges of 3D-Paralleism
				Our solutions
			
		Inference Optimized MoE (Ammar)
			Bring from the blog and our current paper
	
	Democratization of large model inference (Tunji, Cheng, Jeff)
		Inference Optimized ZeRO-Infinity
		
\end{comment}

==> moe-performance.tex <==
\subsection{Performance Evaluation of \moe Inference}
\label{subsec:moe-perf}

In this section, we explore how two broad goals of \textit{high throughput} and \textit{low latency} can be realized for MoE model inference at scale. We also explore how MoE model inference is different compared to their dense counterparts. Model configurations are shown in~\tref{t:inference-table}. 


\begin{table*}[htbp]
% \vskip -0.5em
\caption{The configuration of different MoE models used for the performance evaluation of \moe inference system. These configurations represent the standard MoE architecture cases, and we also test the case of PR-MoE and PR-MoE+MoS, which will have smaller sizes but same (projected) quality.}
\footnotesize
% \vskip -0.5em
\label{t:inference-table}
% \vskip -0.5em
\centering
\begin{tabular}{rcccccccc}
\hline
 {Model} &  {Size (billions)}&  {\#Layers}&  {Hidden size}&  {MP degree} & {EP degree} & {Expert-slicing} & {\#GPUs}\\
\hline
 {1.3B+MoE-128} &  52& 24& 2048 & 1 & 128 & 1 & 128\\
 \hline
 {2.4B+MoE-128} &  107.7& 16& 3584 & 1 & 128 & 1 & 128\\
\hline
 {8B+MoE-128} &  349.0&  30&  4096  &  4&  128 & 1 & 128\\
\hline
 {24B+MoE-128} &  1064.9&  40&  8192&  8 &  128 & 2 & 256\\
\hline
 {47B+MoE-128} &  2024.0&  58&  8192&  8 &  128 & 2 & 256\\
\hline
\end{tabular}
%\vskip -1.5em
\end{table*}

\noindent \textbf{Low-latency and super-linear throughput increase simultaneously:} We scale a 52B MoE model (1.3B base model and 128 experts) from 8 GPUs to 64 GPUs and observe the latency and throughput trends on \moe inference system comparing with a strong baseline, a full-featured distributed PyTorch implementation that is capable of both tensor-slicing and expert-parallelism~\cite{deepspeed-moe-paper}. \fref{fig:latency_tput} shows that both \moe and PyTorch reduce the inference latency as we increase the number of GPUs, as expected, although PyTorch is much slower compared to \moe. Furthermore, \moe obtains increased throughput per GPU when we increase the number of GPUs from 8 to 64 and hence a super-linear increase in total throughput as shown in~\fref{fig:latency_tput}. This is in stark contrast to dense models (best case throughput scaling is linear with respect to the number of GPUs) and shows the major benefit of scaling MoE models over dense models. 

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{figures/moe/1.3B_1.pdf}
\caption{Latency and throughput improvement offered by \moe inference system (Optimized) over PyTorch (Baseline) for a 52-Billion standard MoE model with 128 experts, using between 8 to 64 GPUs.}
\label{fig:latency_tput}
%%\vspace{-0.5cm}
\end{figure}



%As mentioned earlier, the best case throughput scaling for a dense model is linear with respect to the number of GPUs. However, our results in Fig.~\ref{fig:latency_tput} show that \moe obtains increased throughput per GPU when we increase the number of GPUs from 8 to 64 and hence a super-linear increase in total throughput. This is in stark contrast to dense models and shows the major benefit of scaling MoE models over dense models. 
%that the worst-case for MoE model inference is linear speedup (the per GPU throughput remains near-constant for PyTorch MoE). For DeepSpeed, we see increased throughput per GPU when we increase the number of GPUs from 8 to 64 and hence a super-linear speedup. This is in stark contrast to dense models and shows the major benefit of MoE models over dense models, in general. 

%Diving a bit deeper, we see two key properties of expert parallelism at play here: 1) when using expert parallelism, the number of experts per GPU decrease as we increase the number of GPUs. E.g. this 52B MoE model has $128$ total experts; if we serve this using $8$ GPUs, we need $16$ experts per GPU, whereas on $64$ GPUs, we only need $2$ experts per GPU. The decrease in experts per GPU is good for data locality as each GPU is now reading less data (needed for expert parameters) from the memory, and 2) the increase in GPUs could cause performance degradation because of the increased communication between experts (all-to-all) that reside on multiple GPUs. These properties of expert parallelism hold true for both PyTorch and \moe. However, \moe is able to exploit the benefit of expert parallelism to their full potential whereas PyTorch is unable to do so. As \moe exploits advanced communication optimizations (Section~\ref{sec:opt-alltoall}), it significantly overcomes the communication bottleneck in expert parallelism. At the same time, it has highly optimized kernels (Section~\ref{sec:opt-kernels}) that enable it to take advantage of the increased data locality when experts per GPU are reduced. Both these major wins over PyTorch make \moe the framework of choice for getting super-linear increase in throughput with massive scaling, achieving low latency and high throughput simultaneously.
%and perhaps the only framework that can cater to the next-generation of AI scale.


%To study the impact of model scale on MoE inference, we now explore MoE models from 107 billion parameters to 2 trillion parameters using PyTorch and \moe in \fref{fig:moe-vs-moe}.

%\begin{itemize}
%    \item 
\noindent \textbf{Low-latency and high-throughput at unprecedented scale:} \fref{fig:moe-vs-moe-new} shows the performance and throughput of two MoE models with one and two trillion parameters. Compared to baseline, \moe achieves up to 7.3x reduction in latency while achieving up to 7.3x higher throughput. By effectively exploiting hundreds of GPUs in parallel, \moe achieves an unprecedented scale for inference at incredibly low latencies - a staggering trillion parameter MoE model can be served under 25ms.
% \zhewei{We have to explain why baseline uses 128GPUs but XYZ-MoE uses 256 GPUs here. Otherwise, it is really weird.} \yuxiong{let's have all using 256.  For PyTorch, just use 2 data parallel copies. \reza{I agree. I think if we use 256 GPUs in the case of baseline, the tput/GPU stays the same since there won't be any communication happening between two parallel copies.}}
    %\item 
%\end{itemize}

\begin{figure}[htbp]
\centering
%%\vspace{-0.1cm}
\includegraphics[width=0.8\columnwidth]{figures/moe/scale_1.pdf}
\caption{Latency/throughput improvement offered by \moe (Optimized) over PyTorch (Baseline).We ran the experiments on 256 GPUs (throughput is reported per GPU).} %for different MoE model sizes (107 billion to 2 trillion parameters). Throughput is reported per GPU.} %We use 128 GPUs for all configurations for baseline, and 128/256 GPUs for \moe (256 GPUs for the trillion-scale models). The throughputs shown here are per GPU and should be multiplied by number of GPUs to get the aggregate throughput of the cluster.}
\label{fig:moe-vs-moe-new}
%%\vspace{-0.5cm}
\end{figure}




%\begin{figure*}[htbp]
%\centering
%\includegraphics[width=0.8\textwidth]{figures/moe/pr-moe-kd11.pdf}
%\caption{Inference latency comparing standard MoE with PR-MoE and PR-MoE+MoS compression on different GPU count and model sizes. Figure title denotes the model size under standard MoE architecture, and the PR-MoE and PR-MoE+MoS have smaller sizes but same quality (projected for the 2 Trillion case).}
%\label{fig:pr-moe-r2}
%\end{figure*}

%For both Figures \ref{fig:pr-moe-r1} and \ref{fig:pr-moe-r2}, we show a comparison of three model variants along with the baseline version (standard MoE on PyTorch): (i) the standard MoE Model denoted by MoE (DeepSpeed), (ii) the PR-MoE (DeepSpeed), and (iii) the PR-MoE+MoS (DeepSpeed). Results show that the PR-MoE+MoS model offers the lowest latency and enables us to serve the model using only 16 GPUs instead of 32 GPUs. 

%\zhewei{remove deepspeed for submission, change the text in figure to ours? so that we do not need to do it multiple times for this submission}

\noindent \textbf{Better latency and throughput than quality-equivalent dense models:} We now show the comparison between two MoE models with their quality-equivalent dense models: (1) a 52 billion-parameter MoE model (1.3B-MoE-128) compared to a 6.7 billion-parameter dense model in~\fref{fig:moe-vs-dense-r1}, and (2) a 1.5 trillion-parameter MoE model compared to a 175 billion-parameter dense model in~\fref{fig:moe-vs-dense-r2}. When using PyTorch, MoE model inference is more expensive and slower compared to its quality-equivalent dense models. %This is true for both model sizes. 
However, the optimizations in \moe reverse this trend and make MoE model inference both faster and cheaper than quality-equivalent dense models. 
This is a critical result: showing the benefit of MoE models over dense models not only on training but also on inference latency and cost, where real-world deployments care the most.



\begin{figure}[htbp]
\centering
% %\vspace{-0.1cm}
\includegraphics[width=\columnwidth]{figures/moe/52b_1.pdf}
\caption{Inference latency comparison of MoE models and the quality-equivalent 6.7 billion-parameter dense model (throughput is reported per GPU). We ran all MoE models on 128 GPUs, while using one GPU for the dense model.}% We use 1 GPU for 6.7 billion-parameter model as it offers the lowest latency. We use 128 GPUs for the MoE models. The quality-equivalence has been verified by experiments presented in the training section. Figure title denotes the model size under standard MoE architecture, and the PR-MoE and PR-MoE+MoS have smaller sizes but same quality.}
\label{fig:moe-vs-dense-r1}
%\vspace{-0.4cm}
\end{figure}
%We also tested the quality-equivalent PR-MoE+MoS model.

%When comparing the results of~\fref{fig:moe-vs-dense-r1} with~\fref{fig:moe-vs-dense-r2}, we observe that the benefits of MoE models over dense models become even larger with the increase of model size. 
%While in ~\fref{fig:moe-vs-dense-r1} the billion-scale PR-MoE+MoS model (served on \moe) is 2.4x faster and cheaper than the 6.7 billion-parameter dense model (served on PyTorch), in~\fref{fig:moe-vs-dense-r2} the trillion-scale PR-MoE+MoS model is 4.5x faster and 9x cheaper than the 175 billion-parameter dense model.
% While the 52 billion-parameter MoE model (served on DeepSpeed-MoE) is 2.4x faster and cheaper than the 6.7 billion-parameter dense model (served on PyTorch), the 1.5 trillion-parameter MoE model is 4.5x faster and 9x cheaper than the 175 billion-parameter dense model. 

\begin{figure}[htbp]
\centering
\includegraphics[width=\columnwidth]{figures/moe/1.5t_1.pdf}
\caption{Measured inference latency comparison of 1.5T MoE models and assumed quality-equivalent 175 billion dense model (throughput is reported per GPU). We ran MoE experiments on 128 and 256 GPUs for Baseline and XYZ-MoE, while using 16 GPU for the dense model.} %We assume the quality equivalence of these two models with the hypothesis that the scaling law of the smaller scale experiments of Fig.~\ref{fig:moe-vs-dense-r1} holds, as well as from the observations of the published literature. Figure title denotes the model size under standard MoE architecture, and the PR-MoE and PR-MoE+MoS have smaller sizes but same projected quality.}
\label{fig:moe-vs-dense-r2}
%\vspace{-0.5cm}
\end{figure}

The benefits increase for larger models because \moe leverages parallelism-coordinated optimization to reduce communication overhead when using tensor-slicing on the non-expert part of the model. Furthermore, we can take advantage of expert-slicing at this scale, which enables us to scale to a higher number of GPUs compared to the PyTorch baseline. We also observe 2x additional improvement in throughput over latency because MoE models can run with half the tensor-slicing degree of the dense model (8-way vs. 16-way) and thus two times higher batch size.
%In addition, for the larger 1.5 trillion-parameter MoE model, we observed 2x additional improvement in throughput over latency as shown in~\fref{fig:moe-vs-dense-r2}. 
%This is because MoE models can run with half the tensor-slicing degree of the dense model (8-way vs. 16-way) and thus two times higher batch size. 
%Overall, \moe delivers up to 4.5x faster and up to 9x cheaper MoE model inference compared to serving quality-equivalent dense models using PyTorch.
With benefits that scale with model size and hardware resources, we believe that MoE models could be crucial to bring the next generation of advances in AI scale.

% \zhewei{The increasing \# GPUs resulting in better latency is not discussed in the current content yet. Please add it somewhere @Reza.} \reza{@Zhewei, I added the figure the beginning of the inference results (figure~\ref{fig:latency_tput}), please take a look.}


==> pipeline_parallelism_performance.tex <==
\subsection{Performance Evaluation of pipeline parallelism}
\begin{figure}[htb]
\centering
\includegraphics[width=\columnwidth]{figures/pp_speedup.pdf}
\caption{Throughput Improvement with Different Pipeline Parallelism Features for 530B Model.}
\label{fig:pp_speedup}
\end{figure}


==> sys-info.tex <==
% !TeX root = ../main.tex

\begin{table*}[ht]
    % \vspace{-5pt}
% 	\setlength{\abovecaptionskip}{0pt}
    \caption{
    Systems used for ZeRO-Inference evaluation.
    }
    % \setlength{\belowcaptionskip}{-13pt}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lcccccccccc} \toprule
       {Name} & {CPUs} & \shortstack{CPU Memory \\ (GB)} & {GPUs} & \shortstack{FP16 Throughput \\ per GPU (TFLOPS)} & \shortstack{GPU Memory \\ (GB)} & \shortstack{GPU Memory \\ Bandwidth (GB/s)}  & \shortstack{CPU-GPU \\ Bandwidth(GB/s)}  & \shortstack{ GPU-GPU \\ Bandwidth(GB/s)} & \shortstack{NVME Memory \\ (TB)} & \shortstack{NVME Read \\ Bandwidth (GB/sec)} \\ \midrule
        DGX A100 & \shortstack{48-core AMD EPYC \\ 7V12 @3.06 GHz} & 1024 & 8x A100 40 GB SXM  & 312 & 40 & 1555	& 32 & 600 & 8 & 6 \\
        \midrule
        DGX2 V100 & \shortstack{24-core Dual Intel Xeon Platinum\\ @2.7 GHz} & 1500 & 16x V100 32 GB SXM  & 125 & 32 & 900	& 32 & 300 & 30 & 28 \\
        \midrule        Lambda A6000 & \shortstack{24-core AMD Threadripper \\ 3960X @3.8 GHz} & 256 & 2x RTX A6000 & 158.4 & 48 & 768 & 32 & 112.5 & 2 & 5.6 \\
        \bottomrule
        \end{tabular}%
    }
    \label{tab:zero-infer-systems}
    % \vspace{-5pt}
\end{table*}



==> zero_inference_tput.tex <==

\begin{figure*}
    \begin{minipage}[c]{0.1\textwidth}
        \centering
        \includegraphics{figures/zero-inference/1xa6000_tput.png}
        \caption{Throughput of massive transformer models using \zinf on a single A6000 GPU.}
    \end{minipage} \hfill
    \begin{minipage}[c]{0.1\textwidth}
        \centering
        \includegraphics{figures/zero-inference/1xa100_tput.png}
        \caption{Throughput of massive transformer models using \zinf on a single A100-40GB GPU.}
    \end{minipage} \hfill
    \begin{minipage}[c]{0.1\textwidth}
        \centering
        \includegraphics{figures/zero-inference/1xv100_tput.png}
        \caption{Throughput of massive transformer models using \zinf on a single V100-32GB GPU.}
    \end{minipage} 
\caption{Creating subfigures in \LaTeX.}
\label{fig:zero_inf_tputs}
\end{figure*}


